CONTRAST: Continual Multi-source Adaptation to Dynamic Distributions

Adapting to dynamic data distributions is a practical yet challenging task. One effective strategy is to use a model ensemble, which leverages the diverse expertise of different models to transfer knowledge to evolving data distributions. However, this approach faces difficulties when the dynamic test distribution is available only in small batches and without access to the original source data. To address the challenge of adapting to dynamic distributions in such practical settings, we propose Continual Multi-source Adaptation to Dynamic Distributions (CONTRAST), a novel method that optimally combines multiple source models to adapt to the dynamic test data. CONTRAST has two distinguishing features. First, it efficiently computes the optimal combination weights to combine the source models to adapt to the test data distribution continuously as a function of time. Second, it identifies which of the source model parameters to update so that only the model which is most correlated to the target data is adapted, leaving the less correlated ones untouched; this mitigates the issue of ``forgetting" the source model parameters by focusing only on the source model that exhibits the strongest correlation with the test batch distribution. Through theoretical analysis we show that the proposed method is able to optimally combine the source models and prioritize updates to the model least prone to forgetting. Experimental analysis on diverse datasets demonstrates that the combination of multiple source models does at least as well as the best source (with hindsight knowledge), and performance does not degrade as the test data distribution changes over time (robust to forgetting).

==> tables/acdc_dynamic_10steps.tex <==
\begin{table*}[]
\scriptsize
\begin{tabular}{l|ccccccccccccccccc}
\hline
Time                & \multicolumn{1}{l}{t} & \multicolumn{1}{l}{------} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}    \\ \hline
Round               & \multicolumn{1}{l}{1} & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{}      & \multicolumn{1}{l}{4} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{}      & \multicolumn{1}{l}{7} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{}      & \multicolumn{1}{l}{10} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{All} \\ \hline
Conditions          & Rain                  & Snow                       & Fog                  & \multicolumn{1}{c|}{Night} & Rain                  & Snow                 & Fog                  & \multicolumn{1}{c|}{Night} & Rain                  & Snow                 & Fog                  & \multicolumn{1}{c|}{Night} & Rain                   & Snow                 & Fog                  & Night                & Mean                    \\ \hline
Tent-Best-Online    & 20.1                  & 21.3                       & 20.4                 & \multicolumn{1}{c|}{11.8}  & 20.1                  & 21.3                 & 20.4                 & \multicolumn{1}{c|}{11.8}  & 20.1                  & 21.3                 & 20.4                 & \multicolumn{1}{c|}{11.8}  & 20.1                   & 21.3                 & 20.4                 & 11.8                 & 18.4                    \\
Tent-Ens-Online     & 22.4                  & 21.6                       & 23.3                 & \multicolumn{1}{c|}{13.1}  & 22.4                  & 21.6                 & 23.3                 & \multicolumn{1}{c|}{13.1}  & 22.4                  & 21.6                 & 23.3                 & \multicolumn{1}{c|}{13.1}  & 22.4                   & 21.6                 & 23.3                 & 13.1                 & 20.1                    \\
MeTa-Online         & 22.1                  & 22.3                       & 23.5                 & \multicolumn{1}{c|}{13.6}  & 22.1                  & 22.3                 & 23.5                 & \multicolumn{1}{c|}{13.6}  & 22.1                  & 22.3                 & 23.5                 & \multicolumn{1}{c|}{13.6}  & 22.1                   & 22.3                 & 23.5                 & 13.6                 & 20.3                    \\
Tent-Best-Continual & 20.1                  & 20.8                       & 22.6                 & \multicolumn{1}{c|}{11.1}  & 15.9                  & 12                   & 16.8                 & \multicolumn{1}{c|}{8.4}   & 15.3                  & 10.8                 & 15.8                 & \multicolumn{1}{c|}{8.42}  & 15.1                   & 10.4                 & 15.3                 & 8.4                  & 14.3                    \\
Tent-Ens-Continual  & 22.4                  & 20.5                       & 24.3                 & \multicolumn{1}{c|}{12.8}  & 15.4                  & 10.2                 & 15.6                 & \multicolumn{1}{c|}{7.7}   & 14.2                  & 9.4                  & 14.1                 & \multicolumn{1}{c|}{7}     & 13.8                   & 9.2                  & 13.6                 & 7.2                  & 13.4                    \\
MeTA                & 22.1                  & 21.4                       & 24.3                 & \multicolumn{1}{c|}{13.4}  & 18.6                  & 15.5                 & 21.4                 & \multicolumn{1}{c|}{10.4}  & 16.7                  & 13.3                 & 19.5                 & \multicolumn{1}{c|}{10.3}  & 16.4                   & 12.9                 & 19.2                 & 10.2                 & 16.8                    \\ \hline
\end{tabular}
\end{table*}

==> tables/cifar100_dynamic.tex <==
\begin{table*}[]
\caption{\textbf{Comparing the issue of forgetting with the baselines on CIFAR-100.}
This table is obtained using a setting similar to Table~\ref{tab:cifar10-dynamic} and demonstrates the same consistent behavior regarding forgetting. (Results in $\%$ accuracy)}
\vskip 0.08in
\centering
\small
\begin{tabular}{l|cccccccccccc|a}
\hline
Time                & \multicolumn{1}{l}{t} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}               & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}               & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{}    \\ \hline
Round               & \multicolumn{1}{l}{1} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{}              & \multicolumn{1}{l}{3} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{}              & \multicolumn{1}{l}{5} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{All} \\ \hline
Conditions          & Clean                 & Snow                 & Fog                  & \multicolumn{1}{c|}{Frost}         & Clean                 & Snow                 & Fog                  & \multicolumn{1}{c|}{Frost}         & Clean                 & Snow                 & Fog                  & Frost                 & Mean                    \\ \hline
Tent-Best-Online    & 64.5                  & 64.1                 & 60.5                 & \multicolumn{1}{c|}{63.7}          & 64.5                  & 64.1                 & 60.5                 & \multicolumn{1}{c|}{63.7}          & 64.5                  & 64.1                 & 60.5                 & 63.7                  & 63.2                    \\
Tent-Ens-Online     & 72.8                  & 70.5                 & 71.1                 & \multicolumn{1}{c|}{71.9}          & 72.8                  & 70.5                 & 71.1                 & \multicolumn{1}{c|}{71.9}          & 72.8                  & 70.5                 & 71.1                 & 71.9                  & 71.6                    \\
MeTa-Online         & \textbf{76.9}         & \textbf{75}          & \textbf{74.2}        & \multicolumn{1}{c|}{\textbf{74.1}} & \textbf{76.9}         & \textbf{75}          & \textbf{74.2}        & \multicolumn{1}{c|}{\textbf{74.1}} & \textbf{76.9}         & \textbf{75}          & \textbf{74.2}        & \textbf{74.1}         & \textbf{75.1}           \\ \hline
Tent-Best & 64.5                  & 56.1                 & 50.5                 & \multicolumn{1}{c|}{45.6}          & 27.4                  & 20                   & 15.1                 & \multicolumn{1}{c|}{8.9}           & 3.4                   & 3.3                  & 3.1                  & 2.3                   & 24                      \\
Tent-Ens  & 72.8                  & 64.2                 & 60.9                 & \multicolumn{1}{c|}{52.1}          & 24.5                  & 17.1                 & 13.8                 & \multicolumn{1}{c|}{8.1}           & 3.1                   & 2.2                  & 2.6                  & 1.9                   & 25.1                    \\
MeTA                & \textbf{76.9}         & \textbf{71.2}        & \textbf{71.7}        & \multicolumn{1}{c|}{\textbf{68.3}} & \textbf{71.5}         & \textbf{68.5}        & \textbf{68.8}        & \multicolumn{1}{c|}{\textbf{66.9}} & \textbf{71.1}         & \textbf{67.7}        & \textbf{66.9}        & \textbf{65.8}         & \textbf{69.3}           \\ \hline
\end{tabular}
\label{tab:cifar100-dynamic}
\vspace{-0.5em}
\end{table*}

==> tables/cifar100_static.tex <==
\begin{table*}[]
\footnotesize
\begin{tabular}{l|cccccccccccclllc}
\cline{1-13} \cline{17-17}
             & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}          &         &          &                           & \multicolumn{1}{l}{} \\ \hline
             & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{}     & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{}     & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{}         &         &          & \multicolumn{1}{l|}{}     & \multicolumn{1}{l}{} \\ \hline
Domains      & GN                   & SN                   & IN                   & \multicolumn{1}{c|}{DB}   & GB                   & MB                   & ZB                   & \multicolumn{1}{c|}{Snow} & Frost                & Fog                  & Brightness           & \multicolumn{1}{c|}{Contrast} & Elastic & Pixelate & JPEG                      & Mean                 \\ \hline
Source Best  &                      &                      &                      & \multicolumn{1}{c|}{}     &                      &                      &                      & \multicolumn{1}{c|}{}     &                      &                      &                      & \multicolumn{1}{c|}{}         &         &          & \multicolumn{1}{l|}{}     &                      \\
Source Worst &                      &                      &                      & \multicolumn{1}{c|}{}     &                      &                      &                      & \multicolumn{1}{c|}{}     &                      &                      &                      & \multicolumn{1}{c|}{}         &         &          & \multicolumn{1}{l|}{}     &                      \\
Tent Best    & 54.4                 & 54.9                 & 41.3                 & \multicolumn{1}{c|}{66.6} & 57.7                 & 63.4                 & 67.1                 & \multicolumn{1}{c|}{69.7} & 69.6                 & 71                   & 68.3                 & \multicolumn{1}{c|}{65.4}     & 61.2    & 66.7     & \multicolumn{1}{l|}{50.4} & 61.8                 \\
Tent Worst   & 44.1                 & 44.4                 & 30.6                 & \multicolumn{1}{c|}{64.2} & 47.3                 & 62.3                 & 65.3                 & \multicolumn{1}{c|}{56.3} & 55.9                 & 56.8                 & 66.7                 & \multicolumn{1}{c|}{53.8}     & 55.5    & 66.9     & \multicolumn{1}{l|}{42.7} & 53.8                 \\
Tent ENS     & 58.1                 & 59.6                 & 45.4                 & \multicolumn{1}{c|}{72.7} & 61.2                 & 70                   & 72.8                 & \multicolumn{1}{c|}{71.5} & 71.1                 & 72                   & 74.7                 & \multicolumn{1}{c|}{69.8}     & 66.1    & 71.2     & \multicolumn{1}{l|}{56.8} & 66.2                 \\
MeTA         & 57.9                 & 58.8                 & 44.8                 & \multicolumn{1}{c|}{72.5} & 61.5                 & 70                   & 72.8                 & \multicolumn{1}{c|}{71.8} & 72.1                 & 72.7                 & 74.7                 & \multicolumn{1}{c|}{70.6}     & 66.3    & 70.6     & \multicolumn{1}{l|}{54.9} & 66.15                \\ \hline
\end{tabular}
\end{table*}

==> tables/cifar10_dynamic.tex <==
\begin{table*}[]
\caption{\textbf{Comparing the issue of forgetting with the baselines on CIFAR-10.}
This table illustrates that over a prolonged cycle of repetitive test distributions, our model exhibits a much slower rate of forgetting compared to the baseline methods. Note that the ``online" methods represent best-case scenarios that require additional domain knowledge, and they serve as upper bounds for their corresponding continuous adaptation counterparts. (Results in $\%$ accuracy)}
\vskip 0.08in
\centering
\small
\begin{tabular}{l|cccccccccccc|a}
\hline
Time                & \multicolumn{1}{l}{t} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}               & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}               & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{}    \\ \hline
Round               & \multicolumn{1}{l}{1} & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{}              & \multicolumn{1}{l}{3} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{}              & \multicolumn{1}{l}{5} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{All} \\ \hline
Conditions          & Clean                 & Snow                       & Fog                  & \multicolumn{1}{c|}{Frost}         & Clean                 & Snow                 & Fog                  & \multicolumn{1}{c|}{Frost}         & Clean                 & Snow                 & Fog                  & Frost                 & Mean                    \\ \hline
Tent-Best-Online    & 89.2                  & 86.4                       & 87.1                 & \multicolumn{1}{c|}{88.8}          & 89.2                  & 86.4                 & 87.1                 & \multicolumn{1}{c|}{88.8}          & 89.2                  & 86.4                 & 87.1                 & 88.8                  & 87.9                    \\
Tent-Ens-Online     & 93.3                  & 89.4                       & 92.3                 & \multicolumn{1}{c|}{90.5}          & 93.3                  & 89.4                 & 92.3                 & \multicolumn{1}{c|}{90.5}          & 93.3                  & 89.4                 & 92.3                 & 90.5                  & 91.4                    \\
MeTa-Online         & \textbf{93.9}         & \textbf{91.7}              & \textbf{93.9}        & \multicolumn{1}{c|}{\textbf{93.4}} & \textbf{93.9}         & \textbf{91.7}        & \textbf{93.9}        & \multicolumn{1}{c|}{\textbf{93.4}} & \textbf{93.9}         & \textbf{91.7}        & \textbf{93.9}        & \textbf{93.4}         & \textbf{93.2}           \\ \hline
Tent-Best & 89.2                  & 78.4                       & 79.8                 & \multicolumn{1}{c|}{69.7}          & 53.1                  & 44.6                 & 48.6                 & \multicolumn{1}{c|}{45.2}          & 39                    & 29.2                 & 30.1                 & 25.5                  & 52.3                    \\
Tent-Ens  & 93.3                  & 84.5                       & 82.2                 & \multicolumn{1}{c|}{76}            & 61.1                  & 53.4                 & 50.5                 & \multicolumn{1}{c|}{46.4}          & 33.8                  & 29.4                 & 29.6                 & 27.4                  & 54.6                    \\
MeTA                & \textbf{93.9}         & \textbf{90.3}              & \textbf{91.8}        & \multicolumn{1}{c|}{\textbf{90.8}} & \textbf{87.8}         & \textbf{90.7}        & \textbf{87.3}        & \multicolumn{1}{c|}{\textbf{87.1}} & \textbf{85.1}         & \textbf{86.2}        & \textbf{86.3}        & \textbf{86.2}         & \textbf{88.7}           \\ \hline
\end{tabular}
\label{tab:cifar10-dynamic}
\vspace{-0.5em}
\end{table*}

==> tables/cifar10_static.tex <==
\begin{table}[]
\footnotesize
\begin{tabular}{l|cccccccccccc|lllc}
\cline{1-13} \cline{17-17}
             & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} &         &          &      & \multicolumn{1}{l}{} \\ \cline{1-13} \cline{17-17} 
             & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{}     & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{}     & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} &         &          &      & \multicolumn{1}{l}{} \\ \cline{1-13} \cline{17-17} 
Domains      & GN                   & SN                   & IN                   & \multicolumn{1}{c|}{DB}   & GB                   & MB                   & ZB                   & \multicolumn{1}{c|}{Snow} & Frost                & Fog                  & Brightness           & Contrast              & Elastic & Pixelate & JPEG & Mean                 \\ \cline{1-13} \cline{17-17} 
Source Best  &                      &                      &                      & \multicolumn{1}{c|}{}     &                      &                      &                      & \multicolumn{1}{c|}{}     &                      &                      &                      &                       &         &          &      &                      \\
Source Worst &                      &                      &                      & \multicolumn{1}{c|}{}     &                      &                      &                      & \multicolumn{1}{c|}{}     &                      &                      &                      &                       &         &          &      &                      \\
Tent Best    & 80.7                 & 81.6                 & 69.6                 & \multicolumn{1}{c|}{89.4} & 81.3                 & 85.9                 & 89.8                 & \multicolumn{1}{c|}{91.4} & 91.1                 & 92.4                 & 91.9                 & 89.8                  & 84.3    & 88.9     & 79.8 & 85.9                 \\
Tent Worst   &                      &                      &                      & \multicolumn{1}{c|}{}     &                      &                      &                      & \multicolumn{1}{c|}{}     &                      &                      &                      &                       &         &          &      &                      \\
Tent ENS     & 83.2                 & 84.1                 & 73.4                 & \multicolumn{1}{c|}{92.0} & 82                   & 90                   & 92.4                 & \multicolumn{1}{c|}{91.9} & 91.5                 & 92.1                 & 93.5                 & 90.8                  & 87      & 90.6     & 83.7 & 87.9                 \\
MeTA         & 82.7                 & 83.7                 & 71.9                 & \multicolumn{1}{c|}{91.8} & 82.3                 & 89.9                 & 92.5                 & \multicolumn{1}{c|}{92.1} & 91.7                 & 92.1                 & 93.7                 & 91.2                  & 87      & 90.4     & 82.8 & 87.7                 \\ \cline{1-13} \cline{17-17} 
\end{tabular}
\end{table}

==> tables/digit_static.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t!]
\caption{\textbf{Results on Digits dataset.} We train the source models using four digit datasets to perform inference on the remaining dataset. The table clearly shows that MeTA outperforms all of the baselines consistently ($\%$ accuracy).}
\vskip 0.08in
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llccccca}
\toprule
\multicolumn{1}{l}{\textbf{Source}} & \textbf{Method} & \textbf{MM} & \textbf{MT} & \textbf{UP} & \textbf{SV} & \textbf{SY} & \textbf{Avg.} \\ \midrule
\multirow{4}{*}{Single}                    & Source-Best  & 52.3          & 97.8          & 83.2          & 81.7          & 93.3          & 81.7  \\
                                           & Source-Worst & 19.5          & 40.6          & 49.7          & 11.5          & 15.2           & 27.3 \\
                                           & Tent-Best    & 54.8          & 97.7          & 83.3          & 85.6          & 93.3          & 83.0 \\
                                           & Tent-Worst   & 15.8           & 53.1            & 58.9          & 9.9           & 14.6          & 30.5 \\
\cmidrule(l){1-8} 
\multicolumn{1}{l}{\multirow{2}{*}{Multi}} & Tent-Ens     & 61.6 & 96.8         & 87.0            & 54.5          & 77.9          & 75.6 \\
\multicolumn{1}{l}{}                       & MeTA         & \textbf{62.5}         & \textbf{98.1} & \textbf{88.8} & \textbf{85.8} & \textbf{93.3} & \textbf{85.7} \\ \cmidrule(l){1-8} 
\end{tabular}%
}
% \vspace{-0.5em}
\label{tab:digit}
\end{table}

==> tables/office-static.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t!]
\caption{\textbf{Results on Office-Home.} We train three source models using three domains in this dataset and use them for inference on the remaining domain under the TTA setting. Our results demonstrate that MeTA consistently outperforms all of the baselines ($\%$ accuracy).}
\vskip 0.08in
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llcccca}
\toprule
\multicolumn{1}{l}{\textbf{Source}} & \textbf{Method} & \textbf{Ar} & \textbf{Cl} & \textbf{Pr} & \textbf{Re} & \textbf{Avg.} \\ \midrule
\multirow{4}{*}{Single}                    & Source-Best  & 57.5          & 41.5          & 70.2         & 64.3        & 58.4\\
                                           & Source-Worst & 38.6          & 35.1           & 53.8        & 56.1          & 45.9\\
                                           & Tent-Best    & 58.6          & 45.7         & 72.1         & 64.0          &  60.1\\
                                           & Tent-Worst   & 42.3           & 39.6            & 53.5          & 57.9           & 48.3\\
\cmidrule(l){1-7} 
\multicolumn{1}{l}{\multirow{2}{*}{Multi}} & Tent-Ens     & 57.5 & 46.7          & 70.6            & 72.6              &  61.8\\
\multicolumn{1}{l}{}                       & MeTA         & \textbf{59.3}          & \textbf{47.5} & \textbf{72.6} & \textbf{72.6}  & \textbf{63.0}  \\ \cmidrule(l){1-7} 
\end{tabular}%
}
\vspace{-0.5em}
\label{tab:office}
\end{table}
